Focus topics for the ECFA study on Higgs / Top / EW factories

In order to stimulate new engagement and trigger some concrete studies in areas where further work would be beneficial towards fully understanding the physics potential of an $e^+e^-$ Higgs / Top / Electroweak factory, we propose to define a set of focus topics. The general reasoning and the proposed topics are described in this document.

==> authors/AuthorAddresses.tex <==
{\footnotesize

\noindent
$^\ciematno$\ciemat\\ 
$^\desyno$\desy\\
$^\cmuno$\cmu\\
$^\infnpadovano$\infnpadova\\
$^\infnpisano$\infnpisa\\
$^\cernno$\cern\\
$^\infnfrascatino$\infnfrascati\\
$^\slacno$\slac\\
$^\triumfno$\triumf\\ 
$^\mitno$\mit\\
$^\tumunichno$\tumunich\\ 
$^\lpnheno$\lpnhe\\
$^\granadano$\granada\\ 
$^\belgradeno$\belgrade\\
$^\minhono$\minho\\
$^\udineno$\udine\\
$^\copenhagenno$\copenhagen\\
$^\wurzburgno$\wurzburg\\
$^\freiburgno$\freiburg\\
$^\louvainno$\louvain\\
$^\romatreno$\romatre\\
$^\pittno$\pitt\\
$^\karlsruheno$\karlsruhe\\ 
$^\coimbrano$\coimbra\\
$^\liplisbonno$\liplisbon\\
$^\uppsalano$\uppsala\\
$^\brownno$\brown\\
$^\hamburgno$\hamburg\\ 
$^\istlisbonno$\istlisbon\\
$^\oxfordno$\oxford\\ 
$^\madridno$\madrid\\
$^\viennano$\vienna\\
$^\valenciano$\valencia\\
$^\kekno$\kek\\
$^\ljubljanano$\ljubljana\\
$^\cambridgeno$\cambridge\\ 
$^\nikhefno$\nikhef\\
$^\mpimunichno$\mpimunich\\ 
$^\inpkrakowno$\inpkrakow\\
$^\edinburghno$\edinburgh\\ 
$^\shenzhenno$\shenzhen\\
$^\berkeleyno$\berkeley\\ 
$^\infnperugiano$\infnperugia\\
$^\apcno$\apc\\
$^\infntriesteno$\infntrieste\\
$^\clermontauvno$\clermontauv\\
$^\southamptonno$\southampton\\ 
$^\manchesterno$\manchester\\
$^\wisconsinno$\wisconsin\\ 
$^\clermontno$\clermont\\
$^\isfahanno$\isfahan\\
$^\infnpaviano$\infnpavia\\
$^\triesteno$\trieste\\
$^\jukrakowno$\jukrakow\\
$^\grazno$\graz\\
$^\lalno$\lal\\
$^\boskovicno$\boskovic\\ 
$^\glasgowno$\glasgow\\
$^\liverpoolno$\liverpool\\
$^\palaiseauno$\palaiseau\\
$^\bonnno$\bonn\\ 
$^\msuno$\msu\\
$^\dresdenno$\dresden\\
$^\lundno$\lund\\
$^\ughentno$\ughent\\
$^\technionno$\technion\\ 
$^\tokyono$\tokyo\\ 
$^\milanono$\milano\\
$^\warwickno$\warwick\\
$^\kansasno$\kansas\\ 
$^\warsawno$\warsaw\\ 
$^\dmlabno$\dmlab\\
}



==> authors/Authors.tex <==
\begin{center}

\noindent
Juan~Alcaraz~Maestre$^\ciematno$,
Juliette~Alimena$^\desyno$,
John~Alison$^\cmuno$,
Patrizia~Azzi$^\infnpadovano$,
Paolo~Azzurri$^\infnpisano$,
Emanuele~Bagnaschi$^{\cernno,\infnfrascatino}$,
Timothy~Barklow$^\slacno$,
Matthew~J.~Basso$^\triumfno$,
Josh~Bendavid$^\mitno$,
Martin~Beneke$^\tumunichno$,
Eli~Ben-Haim$^\lpnheno$,
Mikael~Berggren$^\desyno$,
Jorge~de~Blas$^\granadano$,
Marzia~Bordone$^\cernno$,
Ivanka~Bozovic$^\belgradeno$,
Valentina~Cairo$^\cernno$,
Nuno~Filipe~Castro$^\minhono$,
Marina~Cobal$^\udineno$,
Paula~Collins$^\cernno$,
Mogens~Dam$^\copenhagenno$,
Valerio~Dao$^\cernno$,
Matteo~Defranchis$^\cernno$,
Ansgar~Denner$^\wurzburgno$,
Stefan~Dittmaier$^\freiburgno$,
Gauthier~Durieux$^\louvainno$,
Ulrich~Einhaus$^\desyno$,
Mary-Cruz~Fouz$^\ciematno$,
Roberto~Franceschini$^\romatreno$,
Ayres~Freitas$^\pittno$,
Frank~Gaede$^\desyno$,
Gerardo~Ganis$^\cernno$,
Pablo~Goldenzweig$^\karlsruheno$,
Ricardo~Gon\c{c}alo$^{\coimbrano,\liplisbonno}$,
Rebeca~Gonzalez~Suarez$^\uppsalano$,
Loukas~Gouskos$^\brownno$,
Alexander~Grohsjean$^\hamburgno$,
Jan~Hajer$^\istlisbonno$,
Chris~Hays$^\oxfordno$,
Sven~Heinemeyer$^\madridno$,
Andr\'e~Hoang$^\viennano$,
Adri\'an~Irles$^\valenciano$,
Abideh~Jafari$^\desyno$,
Karl~Jakobs$^\freiburgno$,
Daniel~Jeans$^\kekno$,
Jernej~F.~Kamenik$^\ljubljanano$,
Matthew~Kenzie$^\cambridgeno$,
Wolfgang~Kilian$^\siegenno$,
Markus~Klute$^\karlsruheno$,
Patrick~Koppenburg$^\nikhefno$,
Sandra~Kortner$^\mpimunichno$,
Karsten~K\"oneke$^\freiburgno$,
Marcin~Kucharczyk$^\inpkrakowno$,
Christos~Leonidopoulos$^\edinburghno$,
Cheng~Li$^\shenzhenno$,
Zoltan~Ligeti$^\berkeleyno$,
Jenny~List$^\desyno$,
Fabio~Maltoni$^\louvainno$,
Elisa~Manoni$^\infnperugiano$,
Giovanni~Marchiori$^\apcno$,
David~Marzocca$^\infntriesteno$,
Andreas~B.~Meyer$^\desyno$,
Ken~Mimasu$^\southamptonno$,
Tristan~Miralles$^\clermontauvno$,
Victor~Miralles$^\manchesterno$,
Abdollah~Mohammadi$^\wisconsinno$,
St\'ephane~Monteil$^\clermontno$,
Gudrid~Moortgat-Pick$^\hamburgno$,
Zohreh~Najafabadi$^\isfahanno$,
Mar\'ia~Teresa~N\'u\~nez~Pardo~de~Vera$^\desyno$,
Fabrizio~Palla$^\infnpisano$,
Michael~E.~Peskin$^\slacno$,
Fulvio~Piccinini$^\infnpaviano$,
Laura~Pintucci$^\triesteno$,
Wies{\l}aw~P{\l}aczek$^\jukrakowno$, 
Simon~Pl\"atzer$^{\grazno,\viennano}$,
Roman~P\"oschl$^\lalno$,
Tania~Robens$^\boskovicno$,
Aidan~Robson$^\glasgowno$,
Philipp~Roloff$^\cernno$,
Nikolaos~Rompotis$^\liverpoolno$,
Andrej~Saibel$^\valenciano$,
Andr\'e~Sailer$^\cernno$,
Roberto~Salerno$^\palaiseauno$,
Matthias~Schott$^\bonnno$,
Reinhard~Schwienhorst$^\msuno$,
Felix~Sefkow$^\desyno$,
Michele~Selvaggi$^\cernno$,
Frank~Siegert$^\dresdenno$, 
Frank~Simon$^\karlsruheno$,
Andrzej~Siodmok$^\jukrakowno$,
Torbj\"orn~Sj\"ostrand$^\lundno$,
Kirill~Skovpen$^\ughentno$,
Maciej~Skrzypek$^\inpkrakowno$,
Yotam~Soreq$^\technionno$,
Raimund~Str\"ohmer$^\wurzburgno$,
Taikan~Suehara$^\tokyono$,
Junping~Tian$^\tokyono$,
Emma~Torro~Pastor$^\valenciano$,
Maria~Ubiali$^\cambridgeno$,
Luiz~Vale~Silva$^\valenciano$,
Caterina~Vernieri$^\slacno$,
Alessandro~Vicini$^\milanono$
Marcel~Vos$^\valenciano$,
Aidan~R.~Wiederhold$^\warwickno$,
Sarah~Louise~Williams$^\cambridgeno$,
Graham~Wilson$^\kansasno$,
Aleksander~Filip~Zarnecki$^\warsawno$,   
Dirk~Zerwas$^{\dmlabno,\lalno}$
\end{center}



